Half-Space Feature Learning in Neural Networks

There currently exist two extreme viewpoints for neural network feature learning -- (i) Neural networks simply implement a kernel method (a la NTK) and hence no features are learned (ii) Neural networks can represent (and hence learn) intricate hierarchical features suitable for the data. We argue in this paper neither interpretation is likely to be correct based on a novel viewpoint. Neural networks can be viewed as a mixture of experts, where each expert corresponds to a (number of layers length) path through a sequence of hidden units. We use this alternate interpretation to motivate a model, called the Deep Linearly Gated Network (DLGN), which sits midway between deep linear networks and ReLU networks. Unlike deep linear networks, the DLGN is capable of learning non-linear features (which are then linearly combined), and unlike ReLU networks these features are ultimately simple -- each feature is effectively an indicator function for a region compactly described as an intersection of (number of layers) half-spaces in the input space. This viewpoint allows for a comprehensive global visualization of features, unlike the local visualizations for neurons based on saliency/activation/gradient maps. Feature learning in DLGNs is shown to happen and the mechanism with which this happens is through learning half-spaces in the input space that contain smooth regions of the target function. Due to the structure of DLGNs, the neurons in later layers are fundamentally the same as those in earlier layers -- they all represent a half-space -- however, the dynamics of gradient descent impart a distinct clustering to the later layer neurons. We hypothesize that ReLU networks also have similar feature learning behaviour.

==> 5_cube_dataset.tex <==
\section{The Cube Dataset}
\label{sec:cube-dataset}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_text_section3.tex <==
We further study the DLGN because they are easy to analyse and interpret because of the disentanglement of linear and non-linear parts in the architecture. We study the behaviour of the overlap kernel deeply and see the effect of different regions of inputs on their structure. \\
Our data set is made up of two different regions which we call them as low frequency and high frequency. We expect to see some structure in the overlap matrix based on the different regions of the input data. The width of the overlap matrix over the slow varying part of the input data should be higher than the high varying part, since any two data points in the slow varying part is more similar than the other part. We confirm this phenomena with the experiments.
\subsection{Link Between Overlap and Neural Tangent Kernel}


\subsection{Problem Setup}
To prove our theory we made a data set, which we call it circle data set. Its label function consists of both low and high frequency which is described below in detail.\\\\
Input Data points are on a $1-sphere$ i.e. $x_i \in S^1$  $ (S^1 = \{x_i \in \mathbb{R}^2 : |x_i| = 1  \})$ equidistant from each other. The dependent variable $y$ is defined such that it is low varying in upper half part of the circle($0^{\circ}$ to $180^{\circ}$) and the high varying part in the lower half part of the circle($180^{\circ}$ to $360^{\circ}$). Mathematically, 

\begin{align*}
    y =
    \begin{cases}
      \sin\{angle\} & \text{if $angle < 180^\circ$} \\
      \sin\{\pi + 9*(angle - \pi \} & \text{if $angle \geq 180^\circ$}\\
    \end{cases}
\end{align*}

% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[scale = .5]{2dcircle.png}
%     \caption{Scatter plot of input data}
    
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[scale = .5]{label_func.png}
%     \caption{Scatter plot of input data}
    
% \end{figure}

\begin{figure}[h]

\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.9\linewidth, scale= .5]{figs/circle/circle.png} 
\caption{Scatter plot of input data}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.9\linewidth,scale = .5]{figs/circle/label_func.png}
\caption{$y$ as a function of angle}
\label{fig:subim2}
\end{subfigure}

\caption{Input Data}
\label{fig:image2}
\end{figure}

\subsection{Dynamics of the Overlap Kernel}
Let $m$ be the number of input data points, $z_l(x)$ denote the output of hidden layer $l$ and let $G_l(x)$ denote the gates of layer $l$. Now, the Kernel for the $i^{t h}$ hidden layer($K_1$) is defined as $K_i(x,x') = \langle G_i(x), G_i(x') \rangle$ where $K_i \in \mathbb{R}^{m x m}$. So the overlap matrix is now $\Lambda = \prod_{i=1}^{i = h} K_i$, where $h$ is number of hidden layers. Basically each entry of overlap matrix or overlap kernel says the number of paths that are active for that the given two inputs.Note that we use overlap matrix or overlap kernel interchangeably. \\\\
In this section, we study and present the dynamics of the overlap kernel for the DLGN with 5 hidden layers, 32 neurons in each layer. MSE is the Loss function used with Adam optimiser with learning rate of 3e-3.\\\\
Figure \ref{fig:overlap_kernels} shows the overlap kernel at different epoch stages. We can see from the figures that the kernel width changes over epochs and at the end of epoch number two the model already decides what kernel width to use for what regions of the input data points. The model recruits low kernel width for the high frequency region and high kernel width for the low frequency region which is clearly visible at the end of last epoch.\\\\
During the learning process of the model, we observed that model first learns low frequency part which happens till epoch number two and later on starts learning the high frequency region which was confirmed by the prediction graphs from Figure \ref{fig:predictions}.

\begin{figure}[h]
\centering
\begin{subfigure}{.3\linewidth}
\includegraphics[ scale= .25]{figs/circle/MLP/loss_epoch.png}
\caption{ReLU}
\label{fig:relu_loss}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
\includegraphics[scale= .25]{figs/circle/both/pwc/DLGN/loss_epoch.png}
\caption{DLGN-BOTH-PWC}
\label{fig:dlgn_both_pwc_loss}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
\includegraphics[ scale= .25]{figs/circle/onpv/pwc/loss_epoch.png}
\caption{DLGN-ONPV-PWC}
\label{fig:dlgn_onpv_pwc_loss}
\end{subfigure}
\caption{Loss v/s Epochs graphs}
\label{fig:circle_loss}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{1\textwidth}
\includegraphics[width=1\linewidth, scale= 2]{figs/circle/MLP/MLP(n_h_l=5,n_n=16,Run=1,Epoch=00000,step=000,UnLearned,train_loss=0.428,train_acc=0.2,test_loss=0.429,test_acc=0.2).png}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\includegraphics[width=1\linewidth, scale= 2]{figs/circle/MLP/MLP(n_h_l=5,n_n=16,Run=1,Epoch=00088,step=008,Learned,train_loss=0.026,train_acc=0.2,test_loss=0.026,test_acc=0.2).png} 
\caption{Kernels at initialization}
\label{fig:subim1}
\end{subfigure}

\begin{subfigure}{1\textwidth}
\includegraphics[width=1\linewidth, scale= 2]{figs/circle/both/pwc/DLGN/DLGN(n_h_l=5,n_n=16,Run=1,Epoch=00000,step=000,UnLearned,train_loss=0.448,train_acc=12.8,test_loss=0.448,test_acc=100.0).png} 
\caption{Kernels at initialization}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\includegraphics[width=1\linewidth, scale= 2]{figs/circle/both/pwc/DLGN/DLGN(n_h_l=5,n_n=16,Run=1,Epoch=00118,step=008,Learned,train_loss=0.009,train_acc=12.8,test_loss=0.009,test_acc=100.0).png} 
\caption{Kernels at initialization}
\label{fig:subim1}
\end{subfigure}

\begin{subfigure}{1\textwidth}
\includegraphics[width=1\linewidth, scale= 2]{figs/circle/onpv/pwc/DLGN(n_h_l=5,n_n=16,Run=1,Epoch=00000,step=000,UnLearned,train_loss=0.445,train_acc=12.8,test_loss=0.445,test_acc=100.0).png} 
\caption{Kernels at initialization}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\includegraphics[width=1\linewidth, scale= 2]{figs/circle/onpv/pwc/DLGN(n_h_l=5,n_n=16,Run=1,Epoch=00500,step=008,Learned,train_loss=0.102,train_acc=12.8,test_loss=0.102,test_acc=100.0).png} 
\caption{Kernels at initialization}
\label{fig:subim1}
\end{subfigure}
\caption{These are the various Kernels visualised as a heat map associated with each hidden layer, the last column(K) being the overlap kernel.During visualisation, the data points(we use 500 data points for circle data set) are sorted in the ascending order from $0^\circ \text{ to } 360^\circ$, hence the first half of the sorted data will consists of low frequency and the other half will consist of high frequencies. Hence the top left region in the overlap kernel is from the low frequency region of the data set and bottom right is from the high frequency region.\\\\}
\label{fig:overlap_kernels}
\end{figure}








% \begin{figure}[h]
% \begin{subfigure}{1\textwidth}
% \centering
% \includegraphics[width=0.9\linewidth, scale= 2]{DLGN(n_h_l = 5, n_n = 32,Run=1,Epoch = 0000,step=00,UnLearned,loss = 0.494).png} 
% \caption{Kernels at initialization}
% \label{fig:subim1}
% \end{subfigure}\\
% \begin{subfigure}{1\textwidth}
% \centering
% \includegraphics[width=0.9\linewidth,scale = 2]{DLGN(n_h_l = 5, n_n = 32,Run=1,Epoch = 0002,step=16,Learned,loss = 0.261).png}
% \caption{Kernels at critical point}
% \label{fig:subim2}
% \end{subfigure}\\
% \begin{subfigure}{1\textwidth}
% \centering
% \includegraphics[width=0.9\linewidth, scale= 2]{DLGN(n_h_l = 5, n_n = 32,Run=1,Epoch = 0040,step=16,Learned,loss = 0.049).png} 
% \caption{Kernel at last epoch}
% \label{fig:subim1}
% \end{subfigure}
% \caption{These are the various Kernels visualised as a heat map associated with each hidden layer, the last column(K) being the overlap kernel.During visualisation, the data points(we use 500 data points for circle data set) are sorted in the ascending order from $0^\circ \text{ to } 360^\circ$, hence the first half of the sorted data will consists of low frequency and the other half will consist of high frequencies. Hence the top left region in the overlap kernel is from the low frequency region of the data set and bottom right is from the high frequency region.\\\\}
% \label{fig:overlap_kernels}
% \end{figure}

% \begin{figure}[h]
% \begin{subfigure}{.5\textwidth}
% \includegraphics[width=0.9\linewidth]{Preds(DLGN, Run=1,Epoch = 0000,step=00,loss = 0.494).png}
% \caption{Predictions at initialization}
% \label{fig:subim1}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
% \includegraphics[width=0.9\linewidth]{Preds(DLGN, Run=1,Epoch = 0002,step=16,loss = 0.261).png}
% \caption{Predictions at critical point}
% \label{fig:subim2}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
% \includegraphics[width=0.9\linewidth]{Preds(DLGN, Run=1,Epoch = 0040,step=16,loss = 0.049).png} 
% \caption{Predictions at last epoch}
% \label{fig:subim1}
% \end{subfigure}
% \caption{Predictions at various epoch stage}
% \label{fig:predictions}
% \end{figure}
% \clearpage
\subsection{Visualizing Active Regions for the DLGN}
Since the data is in 2 dimension, it is possible to visualise and study the hyperplanes associated with all the neurons of all the hidden layers in the model. \\
Let $x_0$ be the input, $x_1, x_2, ..$ be the output of the first, second hidden layer and so on. Let $W_i, b_i$ be weights of the $i^{th}$ hidden layer then,\\

    Hyperplanes for first hidden layer  : $W_1x_0 + b_1 = 0$\\
    Hyperplanes for second hidden layer : $W_2x_1 + b_2 = 0 \Rightarrow W_2(W_1x_0 + b_1) + b_2 = 0$, and so on\\

The blue shaded region is the active regions(for example : $W_1x_0 + b_1 > 0$ for $1^{st}$ hidden layer) i.e. the input regions that lie in the blue shaded region are active for that particular neuron.
\begin{figure}[h]
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[width=.7\linewidth, scale= 1]{figs/circle/both/pwc/Hyperplanes DLGN, , Run = 1, Epoch = 00000, Step = 000.png}
\caption{Hyperplanes at initialization}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[width=.7\linewidth]{figs/circle/both/pwc/Hyperplanes DLGN, , Run = 1, Epoch = 00118, Step = 008.png}
\caption{Hyperplanes at last epoch}
\label{fig:subim2}
\end{subfigure}
\caption{Hyperplanes associated with all the 16 neurons for 5 hidden layers for circle data set.}
\label{fig:image2}
\end{figure}


\begin{figure}[h]
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[width=.7\linewidth]{figs/box/both/pwc/Hyperplanes DLGN, , Run = 1, Epoch = 00000, Step = 000.png}
\caption{Hyperplanes at initialization}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[width=.7\linewidth]{figs/box/both/pwc/Hyperplanes DLGN, , Run = 1, Epoch = 00150, Step = 016.png}
\caption{Hyperplanes at last epoch}
\label{fig:subim2}
\end{subfigure}
\caption{Hyperplanes associated with all the 16 neurons for 5 hidden layers for box data set for BOTH regime}
\label{fig:image2}
\end{figure}

\begin{figure}[h]
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[width=.7\linewidth]{figs/box/onpf/pwc/Hyperplanes DLGN, , Run = 1, Epoch = 00000, Step = 000.png}
\caption{Hyperplanes at initialization}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{1\textwidth}
\centering
\includegraphics[width=.7\linewidth]{figs/box/onpf/pwc/Hyperplanes DLGN, , Run = 1, Epoch = 04000, Step = 016.png}
\caption{Hyperplanes at last epoch}
\label{fig:subim2}
\end{subfigure}
\caption{Hyperplanes associated with all the 16 neurons for 5 hidden layers for box data set for ONPF regime.}
\label{fig:image2}
\end{figure}
\clearpage
\newpage



